OpenCBS: An Open-Source COBOL Defects Benchmark Suite

As the current COBOL workforce retires, entry-level developers are left to keep complex legacy systems maintained and operational. This creates a massive gap in knowledge and ability as companies are having their veteran developers replaced with a new, inexperienced workforce. Additionally, the lack of COBOL and mainframe technology in the current academic curriculum further increases the learning curve for this new generation of developers. These issues are becoming even more pressing due to the business-critical nature of these systems, which makes migrating or replacing the mainframe and COBOL anytime soon very unlikely. As a result, there is now a huge need for tools and resources to increase new developers' code comprehension and ability to perform routine tasks such as debugging and defect location. Extensive work has been done in the software engineering field on the creation of such resources. However, the proprietary nature of COBOL and mainframe systems has restricted the amount of work and the number of open-source tools available for this domain. To address this issue, our work leverages the publicly available technical forum data to build an open-source collection of COBOL programs embodying issues/defects faced by COBOL developers. These programs were reconstructed and organized in a benchmark suite to facilitate the testing of developer tools. Our goal is to provide an open-source COBOL benchmark and testing suite that encourage community contribution and serve as a resource for researchers and tool-smiths in this domain.

==> tex/COBOL_slicing.tex <==
\begin{figure}[ht!]
\begin{minipage}{\linewidth}
\begin{minted}
[
baselinestretch=1,
fontsize=\footnotesize,
]
{cobol}
00001 PROCEDURE DIVISION.
00002 Begin.
00003   OPEN INPUT StudentFile
00004   READ StudentFile
00005     AT END SET EndOfStudentFile TO TRUE
00006   END-READ
00007   PERFORM UNTIL EndOfStudentFile
00008     DISPLAY StudentId 
00009     READ StudentFile
00010        AT END SET EndOfStudentFile TO TRUE
00011     END-READ
00012   END-PERFORM
00013   CLOSE StudentFile
00014   STOP RUN.
\end{minted}
\end{minipage}
\caption{An example of program slicing.}
\end{figure}

==> tex/FESO.tex <==
\begin{figure}
\centering
\includegraphics[width=\linewidth]{figures/FESO.png}
\caption{{\color{red} PLACEHOLDER (REPLACE WITH CORRECT GRAPHICS)} Key concepts 
in the Foreign Exchange Subontology.}
\label{fig:feso_sample}
\end{figure}

==> tex/MISO.tex <==
\begin{figure}
\centering
\includegraphics[width=\linewidth]{figures/MISO.png}
\caption{{\color{red} PLACEHOLDER (REPLACE WITH CORRECT GRAPHICS)} Key concepts 
in the micro-banking subontology. Figure~\ref{fig:miso_sample}(a) shows the 
components of \concept{Action} and Figure~\ref{fig:miso_sample}(b) shows the 
componenets of \concept{Intangible}.}
\label{fig:miso_sample}
\end{figure}
